Multidimensional Butterfly Factorization

This paper introduces the multidimensional butterfly factorization as a data-sparse representation of multidimensional kernel matrices that satisfy the complementary low-rank property. This factorization approximates such a kernel matrix of size $N\times N$ with a product of $\O(\log N)$ sparse matrices, each of which contains $\O(N)$ nonzero entries. We also propose efficient algorithms for constructing this factorization when either (i) a fast algorithm for applying the kernel matrix and its adjoint is available or (ii) every entry of the kernel matrix can be evaluated in $\O(1)$ operations. For the kernel matrices of multidimensional Fourier integral operators, for which the complementary low-rank property is not satisfied due to a singularity at the origin, we extend this factorization by combining it with either a polar coordinate transformation or a multiscale decomposition of the integration domain to overcome the singularity. Numerical results are provided to demonstrate the efficiency of the proposed algorithms.

==> figure/fig-comp-modules/fig-comp-h.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,4,...,12}{
\foreach \i in {0,1,...,3} {
    \draw[fill=lightgray] (\k+\i,16-\k) rectangle (\k+\i+1,12-\k);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,4,...,12}{
\foreach \i in {0,1,...,3} {
    \draw[fill=gray] (\k+\i,16-\i-\k) rectangle (\k+\i+1,16-\i-\k-1);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-compression-2DV.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v2}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-v}
}\\
\end{minipage}
\caption{The recursive factorization $(V^2)^* \approx (H^2)^*(V^3)^*$ of $(V^2)^*$
    in Figure~\ref{fig:compression-2D}.}
\label{fig:compression-1D3}
\end{figure}

